Reconstructive Visual Instruction Tuning

This paper introduces reconstructive visual instruction tuning (ROSS), a family of Large Multimodal Models (LMMs) that exploit vision-centric supervision signals. In contrast to conventional visual instruction tuning approaches that exclusively supervise text outputs, ROSS prompts LMMs to supervise visual outputs via reconstructing input images. By doing so, it capitalizes on the inherent richness and detail present within input images themselves, which are often lost in pure text supervision. However, producing meaningful feedback from natural images is challenging due to the heavy spatial redundancy of visual signals. To address this issue, ROSS employs a denoising objective to reconstruct latent representations of input images, avoiding directly regressing exact raw RGB values. This intrinsic activation design inherently encourages LMMs to maintain image detail, thereby enhancing their fine-grained comprehension capabilities and reducing hallucinations. Empirically, ROSS consistently brings significant improvements across different visual encoders and language models. In comparison with extrinsic assistance state-of-the-art alternatives that aggregate multiple visual experts, ROSS delivers competitive performance with a single SigLIP visual encoder, demonstrating the efficacy of our vision-centric supervision tailored for visual outputs.

==> sections/7.rebuttal.tex <==
\section{Summary of Revisions}

We sincerely thank all reviewers for their valuable and constructive comments.
%
We have tried our best to revise the paper to address all concerns. 
%
\textit{All revisions are marked in purple.}
%
Specifically:

\begin{itemize}
    \item \textbf{@Reviewer kvNB}, \textbf{Reviewer SsLG}, and \textbf{Reviewer rXNr}, we have added discussions on computational costs in Section 5.2 and detailed comparisons at Table 10 in Appendix B, where our Ross brings marginal computational overhead.

    \item \textbf{@Reviewer SsLG}, to better illustrate our insight, we have provided reconstruction results in Figure 9 in Section 5.2, where high-level features of Ross-7B can be projected back into the pixel space.

    \item \textbf{@Reviewer SsLG}, we have provided an ablation on the schedule of $\beta$ in Table 11 in Appendix C.1, where our Ross is robust against different denoising schedules.

    \item \textbf{@Reviewer MCFE} and \textbf{Reviewer rXNr}, we have provided a more comprehensive A/B experiment in Table 12 in Appendix C.1, where the proposed vision-centric objective brings significant improvements in most cases.

    \item \textbf{@Reviewer MCFE}, we have incorporated the ``anyres'' technique and compared state-of-the-art alternatives on high-resolution benchmarks in Table 13 in Appendix C.2, where our Ross-7B-anyres surpasses LLaVA-v1.6-7B and Cambrian-1-8B under most cases.

    \item \textbf{@Reviewer tGMa}, we have studied the impact of Ross on language capabilities in Table 14 in Appendix C.3, where Ross does not harm language capabilities as it brings improvements in most cases.

    \item \textbf{@Reviewer tGMa}, we have investigated the effectiveness of Ross across different model sizes in Table 15 in Appendix C.3, where Ross brings improvements over the baseline (LLaVA) across different model sizes in most cases.

    \item \textbf{@Reviewer kvNb} and \textbf{Reviewer tGMa}, we have studied the data scaling property of our Ross in Table 16 in Appendix C.3, where Ross consistently brings significant improvements as the training data scale increases.

    \item \textbf{@Reviewer tGMa}, to better explain the reasoning behind how the vison-centric supervision enables the model to focus on relevant areas, we visualize the gradient using GradCAM in Figure 12 in Appendix C.3, where Ross generates reasonable gradients as training evolves, guiding the model to focus on the relevant regions of the image.

\end{itemize}


Please let us know if you have any further questions.
%
We are always looking forward to open discussions.


Sincerely,

Authors






\section{{To Reviewer kvNb (1)}}


We thank reviewer kvNb for the valuable time and constructive feedback. 
%
We are truly grateful for your use of the terms ``novel'' and ``makes sense'' to describe our work.
%
Your appreciation of our comprehensive analysis and the robust empirical validation is greatly encouraging.
%
Point-to-point responses are provided below.


\textbf{W1: Potential Unfairness in Comparisons.} While the paper includes an ablation study where variables like training data are controlled for fair comparison with other models, its main results table appears to use different datasets compared to competing methods. This inconsistency in data setup might lead to an unfair advantage for Ross, making it difficult to assess the true comparative effectiveness of the approach against state-of-the-art methods.


\textbf{A1:}
We appreciate the reviewer's concern regarding the potential unfairness in the comparisons presented in Table 4.
%
We have tried our best to conduct fair comparisons against the baseline, including the same visual encoder, base language model, pre-training and instruction tuning data, where significant improvements are observed consistently, which can be found in Table 3.
%
We acknowledge that the comparisons in Table 4 might be perceived as unfair due to the use of different datasets.
%
To mitigate this concern, we have performed an additional experiment where we compare Ross with the state-of-the-art method, LLaVA, using the exact same datasets and settings. 
%
Specifically, we used the CLIP-ViT-L/14@336 visual encoder and the Qwen2-7B-Instruct language model. 
%
Empirical results below demonstrate that Ross consistently outperforms LLaVA under these identical conditions.

\begin{table}[H]
    \centering\small
    \vspace{-5pt}
    \begin{tabular}{llc llllll}
    \toprule
    PT & SFT & $\mathcal{L}_{\mathrm{LMM}}^{\mathrm{visual}}$ & POPE & Hallu. & ChartQA & OCRBench & MMB$^{\text{EN}}$ & AI2D \\
    
    \midrule
    \multirow{2}{*}{558K} & \multirow{2}{*}{737K} & -- & 87.9 & 55.0 & 34.0 & 363 & 73.8 & 72.4 \\
    & & \checkmark & \textbf{88.4 \up{0.5}} & \textbf{59.1 \up{4.1}} & \textbf{40.4 \up{6.4}} & \textbf{380 \up{17}} & \textbf{75.2 \up{1.4}} & \textbf{73.3 \up{0.9}} \\

    \midrule
    \multirow{2}{*}{2M} & \multirow{2}{*}{1.2M} & -- & 88.5 & 53.8 & 41.2 & 388 & 76.5 & 73.9 \\
    & & \checkmark & \textbf{88.9 \up{0.4}} & \textbf{57.3 \up{2.5}} & \textbf{43.2 \up{2.0}} & \textbf{405 \up{17}} & \textbf{78.0 \up{1.5}} & \textbf{74.1 \up{0.2}} \\
    
    \bottomrule
    \end{tabular}
\end{table}


We acknowledge that the comparison in Table 4 might be unfair, which is actually a common problem in the field of LMMs as there are many challenges in conducting fully fair comparisons.
%
We have listed a series of representative components that lead to this unfairness in the following table.
%
It was relatively hard for researchers to conduct a completely fair comparison against the state-of-the-art methods, not to mention that some methods may contribute at the data level, \textit{e.g.}, ShareGPT4V.


\begin{table}[H]
    \centering\footnotesize
    \begin{tabular}{llcclll}
    \toprule
    Method & Encoder & Resolution & \# tokens & LLM & Pre-train & SFT \\
    \midrule
    LLaVA-v1.5-7B & CLIP-L/14 & 336 & & Vicuna-7B-v1.5 & 558K & 665K \\
    
    LLaVA-v1.6-7B & CLIP-L/14 & 5$\times$336 & 5$\times$576 & Vicuna-7B-v1.5 & 558K & 665K \\

    \multirow{2}{*}{Mini-Gemini-7B} & CLIP-L/14 & 336 & \multirow{2}{*}{576} & \multirow{2}{*}{Mixtral-8x7B} & \multirow{2}{*}{1.2M} & \multirow{2}{*}{1.5M} \\
    & + ConvNeXt-L & 768 \\
    
    \multirow{4}{*}{Cambrian-1-8B} & CLIP-L/14 & 336 & \multirow{4}{*}{576} & \multirow{4}{*}{Llama3-8B-Instruct} & \multirow{4}{*}{2.5M} & \multirow{4}{*}{7M} \\
    & + SigLIP-L/14 & 384 \\
    & + DINOv2-L/14 & 518 \\
    & + ConvNeXt-XXL & 1024 \\
    
    Ross-7B & SigLIP-L/14 & 384 & 729 & Qwen2-7B-Instruct & 2M & 1.2M \\
    \bottomrule
    \end{tabular}
\end{table}






\textbf{W2: Computational Overhead.} The denoising process introduces extra computational overhead during training, but the paper does not quantify or discuss this cost, leaving readers uncertain about the practical trade-offs of using this approach.


\textbf{A2:}
We apologize for the oversight in quantifying and discussing the computational overhead introduced by the denoising process. 
%
To address this concern, we have conducted additional experiments to measure the computational costs and provide a clearer understanding of the practical trade-offs.
%
Evaluations are conducted using 8 A100 GPUs with a global batch size of 128.
%
Due to the limited GPU memory, we accumulate 4 gradient steps and the batch size per GPU is 4.
%
The whole stage requires 5757 training steps.
%
GPU memories are averaged over 8 GPUs with DeepSpeed Zero 3.
%
As demonstrated in the following table, the denoising process introduces a negligible increase in training time ($\approx$10\% compared to the baseline), while the benefits outweigh the minor additional costs.


\begin{table}[H]
    \centering\small
    % \caption{
    % \textbf{Comparisons on computational costs during the instruction tuning stage} with Cambrian-737K~\citep{tong2024cambrian}, where evaluations are conducted using 8 A100 GPUs with a global batch size of 128.
    % %
    % Due to the limited GPU memory, we accumulate 4 gradient steps and the batch size per GPU is 4.
    % %
    % The whole stage requires 5757 training steps.
    % %
    % GPU memories are averaged over 8 GPUs with DeepSpeed Zero 3.
    % }
    % \label{tab:cost}
    \vspace{-5pt}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{ll c lllll}
    \toprule
    Vision & Base LLM & $\mathcal{L}_{\mathrm{LMM}}^{\mathrm{visual}}$ & \begin{tabular}[c]{@{}l@{}}Trainable\\ Parameters\end{tabular} & Speed (s/iter) & Time & \begin{tabular}[c]{@{}l@{}}GPU\\ Memory\end{tabular} \\
    \midrule
    CLIP-L/336 & Qwen2-7B-Instruct & -- & 7.63 B & 8.31 & 13h 17min & 45.34 G \\
    CLIP-L/336 & Qwen2-7B-Instruct & \checkmark & 7.68 B & 9.02 (1.09$\times$) & 14h 25min & 46.62 G (1.03$\times$) \\

    CLIP-L/336 & Vicuna-13B-v1.5 & -- & 13.05 B & 13.33 & 21h 19min & 48.62 G \\
    CLIP-L/336 & Vicuna-13B-v1.5 & \checkmark & 13.11 B & 14.69 (1.10$\times$) & 23h 30min & 49.07 G (1.01$\times$) \\

    \midrule

    SigLIP-L/384 & Qwen2-7B-Instruct & -- & 7.63 B & 8.77 & 14h 1min & 47.08 G \\
    SigLIP-L/384 & Qwen2-7B-Instruct & \checkmark & 7.68 B & 9.48 (1.08$\times$) & 15h 9min & 52.07 G (1.11$\times$) \\

    SigLIP-L/384 & Vicuna-13B-v1.5 & -- & 13.05 B & 14.22 & 22h 44min & 48.80 G \\
    SigLIP-L/384 & Vicuna-13B-v1.5 & \checkmark & 13.11 B & 15.32 (1.08$\times$) & 24h 30min & 52.68 G (1.08$\times$) \\
    \bottomrule
    \end{tabular}
\end{table}



\textbf{W3: Limited Analysis of Generation vs. Reconstruction Performance.} The paper compares Ross’s reconstructive approach to generative methods, noting that the generative approach underperforms in comprehension tasks. However, it lacks a thorough exploration of why the generative method yields lower performance. A more in-depth discussion of the limitations and differences between the two approaches would enhance understanding and help identify when reconstruction might be preferable to generation in multimodal tasks.


\textbf{A3:}
% First, we would like to clarify that most generative methods, such as Chameleon and Show-o, aim to equip both comprehension and creation within a \textit{single} model, which often underperforms in comprehension tasks.
%
We hypothesize that the underlying reason for the lower performance of generative methods in comprehension tasks is \textit{the weak correspondence between inputs and supervision} under generative settings, which typically arises from both the (1) data and the (2) design of these methods.

(1) Typical generative methods that explore the synergy of comprehension and generation, usually leverage image generation conditioned on text instructions on \textit{(i) text-to-image datasets} or \textit{(ii) interleaved datasets} as extra supervision.
%
However, (i) text-to-image datasets are typically designed to generate \textit{high-aesthetic} samples rather than text-aligned ones, and (ii) interleaved datasets aim to enable few-shot learning via interleaving independent supervised examples, where reasoning becomes more important than alignment.
%
Therefore, there exists a clear disconnect where the supervision (image) has little to do with the input (text instruction).
%
For example, the CLIP-Score~\citep{hessel2021clipscore}, which measures the similarity between text and images, is only 0.3043 for the LAION-Art dataset~\citep{schuhmann2022laion} and 0.2842 for the MMC4 dataset~\citep{zhu2023multimodal}, indicating that the supervision signals in these datasets are \textit{not} well-suited for tasks requiring strong text-image alignment.


(2) Even when we attempt to ensure image-text alignment by converting aligned caption data into creation data for supervision, the results demonstrated in Table 2 remain unsatisfactory.
%
This suggests that the \textit{design of generative objectives itself does not inherently require a strong correspondence} between inputs and supervision targets.

In contrast, reconstructive methods like Ross leverage the original input images as auxiliary supervision, ensuring a strong and direct correspondence, which is crucial for tasks requiring accurate comprehension and interpretation of multimodal data, leading to significantly improved performance.












\section{{To Reviewer MCFE (2)}}


We thank Reviewer MCFE very much for the insightful feedback. 
%
We are particularly grateful for your acknowledgment of the ``step forward'' our technique represents. 
%
Your recognition of the ``significant'' improvements in metrics is highly encouraging. 
%
Point-to-point responses are provided below.


\textbf{W1: Clean A/B Experiment with Extended Evaluation Benchmarks.} I wish the benchmarks cited in the paper to measure the benefits of their method, I wish those benchmarks more closely matched recent popular work such as "The Llama 3 Herd of Models" or "Qwen2-VL", which include benchmarks like TextVQA, DocVQA, etc ... It may not change the conclusion but when we compare methods, it's important to look at a representative distribution of benchmarks. Table 4 has some of these common benchmarks, but not all of them. Furthermore, I wish Table 4 (or perhaps Table 3) included the same benchmarks but also had a very clean A/B experiment that was a baseline without the method vs. using the method. Table 3 has this but Table 3 has a different set of benchmarks! So it's rather confusing what conclusion to draw.


\textbf{A1:}
We apologize that the provided A/B experiment in Table 3 is not comprehensive enough.
%
Following your suggestion, we extend the  A/B experiment in Table 3 by incorporating more benchmarks such as TextVQA and DocVQA, providing a more balanced and representative distribution of tasks, where scores of OCRBench are divided by 10 for computing averaged scores.


Empirical results in the following table demonstrate that our proposed vision-centric supervision utilized by Ross leads to significant improvements in most cases.
%
Moreover, we found Ross contributes more significant improvements over fine-grained comprehension datasets, such as HallusionBench, MMVP, ChartQA, and OCRBench.




\begin{table}[H]
    \centering\footnotesize
    % \caption{
    % \textbf{Extended ablations.}
    % }
    % \label{tab:complete_abl}
    \vspace{-5pt}
    \setlength{\tabcolsep}{3pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l rr rr rr rr}
    \toprule
    & \multicolumn{4}{c}{CLIP-ViT-L/14@336} & \multicolumn{4}{c}{SigLIP-ViT-SO400M/14@384} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    & \multicolumn{2}{c}{Vicuna-7B-v1.5} & \multicolumn{2}{c}{Qwen2-7B-Instruct} & \multicolumn{2}{c}{Vicuna-7B-v1.5} & \multicolumn{2}{c}{Qwen2-7B-Instruct} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    Benchmark & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} \\
    \midrule
    
    POPE$_{\text{acc}}$ & 86.3 & \textbf{87.2 \up{0.9}} & 87.9 & \textbf{88.4 \up{0.5}} & 86.0 & \textbf{87.7 \up{1.7}} & 88.5 & \textbf{88.7 \up{0.2}} \\
    
    HallusionBench$_{\text{aAcc}}$ & 52.5 & \textbf{55.8 \up{3.3}} & 55.0 & \textbf{59.1 \up{4.1}} & 50.4 & \textbf{53.8 \up{3.4}} & 57.3 & \textbf{58.2 \up{0.9}} \\
    
    MMBench-EN$_{\text{dev}}$ & 67.0 & \textbf{67.6 \up{0.6}} & 73.8 & \textbf{75.2 \up{1.4}} & 64.5 & \textbf{69.2 \up{4.7}} & 76.3 & \textbf{76.9 \up{0.6}} \\
    
    MMBench-CN$_{\text{dev}}$ & \textbf{60.0} & 59.8 \down{0.2} & 72.9 & \textbf{73.7 \up{0.8}} & 63.1 & \textbf{63.4 \up{0.3}} & 75.7 & \textbf{76.3 \up{0.7}} \\
    
    SEED$_{\text{img}}$ & \textbf{66.7} & 66.4 \down{0.3} & 70.3 & \textbf{70.7 \up{0.4}} & 68.2 & \textbf{69.0 \up{0.8}} & \textbf{72.3} & 72.1 \down{0.2} \\
    
    MMMU$_{\text{dev}}$ & 30.0 & \textbf{34.0 \up{4.0}} & 44.0 & \textbf{45.3 \up{1.3}} & 33.3 & \textbf{38.0 \up{4.7}} & 38.7 & \textbf{41.3 \up{2.6}} \\
    
    MMMU$_{\text{val}}$ & 35.3 & \textbf{36.0 \up{0.7}} & 41.9 & \textbf{42.6 \up{0.7}} & 34.2 & \textbf{35.4 \up{1.2}} & 41.8 & \textbf{43.8 \up{2.0}} \\
    
    MMVP & 28.0 & \textbf{36.3 \up{8.3}} & 29.6 & \textbf{42.2 \up{12.6}} & 27.3 & \textbf{38.0 \up{10.7}} & 40.7 & \textbf{49.3 \up{8.6}} \\
    
    AI2D$_{\text{test}}$ & 61.2 & \textbf{61.4 \up{0.2}} & 71.9 & \textbf{73.3 \up{1.4}} & \textbf{62.6} & 62.4 \down{0.2} & 74.0 & \textbf{74.5 \up{0.5}} \\
    
    ChartQA$_{\text{test}}$ & 32.9 & \textbf{39.8 \up{6.9}} & 36.2 & \textbf{41.6 \up{5.4}} & 34.0 & \textbf{48.2 \up{14.2}} & 44.4 & \textbf{46.9 \up{2.5}} \\
    
    DocVQA$_{\text{val}}$ & 33.4 & \textbf{41.6 \up{8.2}} & 31.1 & \textbf{44.7 \up{13.6}} & 40.4 & \textbf{40.7 \up{0.3}} & 39.2 & \textbf{39.3 \up{0.1}} \\
    
    InfoVQA$_{\text{val}}$ & 21.2 & \textbf{26.4 \up{5.2}} & 22.1 & \textbf{39.3 \up{16.2}} & 22.8 & \textbf{23.3 \up{0.5}} & 24.0 & \textbf{25.1 \up{1.1}} \\
    
    TextVQA$_{\text{val}}$ & 55.7 & \textbf{58.7 \up{3.0}} & 52.0 & \textbf{54.1 \up{2.1}} & 60.5 & \textbf{62.6 \up{2.1}} & 56.3 & \textbf{57.5 \up{1.2}} \\
    
    OCRBench & 339 & \textbf{350 \up{11}} & 363 & \textbf{381 \up{18}} & 354 & \textbf{365 \up{11}} & 432 & \textbf{448 \up{16}} \\
    
    RealWorldQA & 52.7 & \textbf{53.2 \up{0.5}} & 56.7 & \textbf{57.4 \up{0.7}} & 55.0 & \textbf{57.1 \up{2.1}} & 57.9 & \textbf{59.1 \up{1.2}} \\

    \cmidrule{1-9}

    Average & 47.8 & \textbf{50.6 \up{2.8}} & 52.1 & \textbf{56.4 \up{4.3}} & 49.2 & \textbf{52.4 \up{3.2}} & 55.4 & \textbf{56.9 \up{1.5}} \\
    
    \bottomrule
    \end{tabular}}
\end{table}



\textbf{W2 \& Q1: Comparison on High-Resolution Benchmarks.} The fact that the work was done at lower image resolution also limits the impact of the work. While it may be a perfectly reasonably thing to study the problem initially at lower resolution, I believe that most people care about the models with the best metrics, and all of those methods today use image tiling to handle high resolution images. How will the results change at higher resolution and what would the comparison look like when compared against tile-based methods like LLava-1.6 or any of the more recent VLM work like Qwen2-VL etc ...?


\textbf{A2:}
We appreciate the feedback regarding the need for high-resolution comparisons.
%
To address this concern, we have incorporated the ``anyres'' technique proposed by LLaVA-v1.6 into our Ross.
%
Specifically, for each image, we employ a grid configuration of 384$\times$\{2$\times$2, 1$\times$\{2,3,4\}, \{2,3,4\}$\times$1\} to identify the input resolution, resulting in a maximum of 5$\times$729 $=$ 3,645 visual tokens.
%
\textit{Each} 384$\times$384 crop is required to reconstruct the original input via the denoising objective proposed by Ross.
%
In the following table, our \textbf{\method-7B}$_{\text{anyres}}$ surpasses LLaVA-v1.6-7B and Cambrian-1-8B under most cases.
%
These results indicate that Ross not only performs well at lower resolutions but also maintains its competitive edge at higher resolutions, making it a robust and versatile method.




\begin{table}[H]
    \centering\small
    % \caption{
    % \textbf{Comparison to state-of-the-art LMMs on benchmarks requires high-resolution inputs.}
    % %
    % We evaluate models on: ChartQA~\citep{masry2022chartqa}, DocVQA~\citep{mathew2021docvqa} val set, InfoVQA~\citep{biten2022infovqa} val set, TextVQA~\citep{singh2019towards} val set, OCRBench~\citep{liu2023ocrbench}, and RealWorldQA~\citep{xai2024grok}.
    % %
    % Evaluations of ChartQA, DocVQA, InfoVQA, and TextVQA are conducted on lmms-eval~\citep{lmmseval2024}, while evaluations of OCRBench and RealWorldQA are conducted with VLMEvalKit~\citep{duan2024vlmevalkit}.
    % %
    % $^\ddag$We evaluate the official checkpoint.
    % }
    % \vspace{-5pt}
    \setlength{\tabcolsep}{3pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{r cccccc}
        \toprule
        Model & ChartQA & DocVQA & InfoVQA & TextVQA  & OCRBench & RealWorldQA\\
        \midrule

        GPT-4V-1106 \citep{gpt4v}  & 78.5 & 88.4 & -- & 78.0 & 645 & 61.4 \\
        Gemini-1.5 Pro \citep{team2023gemini} & 81.3 & 86.5 & -- & 78.1 & -- & 67.5 \\
        Grok-1.5 \citep{xai2024grok} & 76.1 & 85.6 & -- & 78.1 & -- & 68.7 \\
            
        \midrule 
        
        LLaVA-v1.5-7B$^\ddag$ \citep{liu2024improved} & 18.2 & 28.1 & 25.7 & 58.2 & 317 & 54.9 \\
        LLaVA-v1.6-7B$^\ddag$ \citep{liu2024llavanext} & 65.5 &  74.4 & 37.1 & 64.8 & 532 & 57.6 \\
        % Mini-Gemini-7B \citep{li2024mini} & 59.1 & 74.6 & -- & 70.2 & 477 & 62.1 \\
        % DeepSeek-VL-7B \citep{lu2024deepseek} \\
        Cambrian-1-8B \citep{tong2024cambrian} & 73.3 & 77.8 & -- & 71.7 & \textbf{624} & 64.2 \\
        
        \textbf{\method-7B}$_{\text{anyres}}$ & \textbf{76.9} & \textbf{81.8} & \textbf{50.5} & \textbf{72.2} & 607 & \textbf{66.2} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:ocr}
\end{table}














\section{{To Reviewer SsLG (3)}}

We thank Reviewer SsLG for the insightful and positive feedback. 
%
We are deeply appreciative of using ``very novel'' and the recognition of the importance of vision-centric learning in LMMs. 
%
The acknowledgment of our ``innovative vision-centric supervision method'' and the ``clever'' use of denoising objectives is highly encouraging.
%
We are also grateful for your praise of our ``extensive experiments'' and ``thorough ablation studies''.
%
We provide point-to-point responses below.

\textbf{W1: Computational Costs.} I think the major weakness is about the Computational Costs. While the paper emphasizes the efficiency of using a single visual encoder, it lacks detailed analysis of training time, memory requirements, and computational costs compared to baseline methods.



\textbf{A1:}
We apologize for the oversight in discussing the computational overhead quantitatively.
%
To address this concern, we have conducted additional experiments in the following table to measure the computational costs and provide a clearer understanding of the practical trade-offs.
%
Evaluations are conducted using 8 A100 GPUs with a global batch size of 128, where the batch size per GPU remains 4 4 gradient steps are accumulated.
%
GPU memories are averaged over 8 GPUs with DeepSpeed Zero 3.
%
As demonstrated in the following table, Ross introduces a marginal increase in training time and GPU memory.




\begin{table}[H]
    \centering\small
    % \caption{
    % \textbf{Comparisons on computational costs during the instruction tuning stage} with Cambrian-737K~\citep{tong2024cambrian}, where evaluations are conducted using 8 A100 GPUs with a global batch size of 128.
    % %
    % Due to the limited GPU memory, we accumulate 4 gradient steps and the batch size per GPU is 4.
    % %
    % The whole stage requires 5757 training steps.
    % %
    % GPU memories are averaged over 8 GPUs with DeepSpeed Zero 3.
    % }
    % \label{tab:cost}
    \vspace{-5pt}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{ll c lllll}
    \toprule
    Vision & Base LLM & $\mathcal{L}_{\mathrm{LMM}}^{\mathrm{visual}}$ & \begin{tabular}[c]{@{}l@{}}Trainable\\ Parameters\end{tabular} & Speed (s/iter) & Time & \begin{tabular}[c]{@{}l@{}}GPU\\ Memory\end{tabular} \\
    \midrule
    CLIP-L/336 & Qwen2-7B-Instruct & -- & 7.63 B & 8.31 & 13h 17min & 45.34 G \\
    CLIP-L/336 & Qwen2-7B-Instruct & \checkmark & 7.68 B & 9.02 (1.09$\times$) & 14h 25min & 46.62 G (1.03$\times$) \\

    CLIP-L/336 & Vicuna-13B-v1.5 & -- & 13.05 B & 13.33 & 21h 19min & 48.62 G \\
    CLIP-L/336 & Vicuna-13B-v1.5 & \checkmark & 13.11 B & 14.69 (1.10$\times$) & 23h 30min & 49.07 G (1.01$\times$) \\

    \midrule

    SigLIP-L/384 & Qwen2-7B-Instruct & -- & 7.63 B & 8.77 & 14h 1min & 47.08 G \\
    SigLIP-L/384 & Qwen2-7B-Instruct & \checkmark & 7.68 B & 9.48 (1.08$\times$) & 15h 9min & 52.07 G (1.11$\times$) \\

    SigLIP-L/384 & Vicuna-13B-v1.5 & -- & 13.05 B & 14.22 & 22h 44min & 48.80 G \\
    SigLIP-L/384 & Vicuna-13B-v1.5 & \checkmark & 13.11 B & 15.32 (1.08$\times$) & 24h 30min & 52.68 G (1.08$\times$) \\
    \bottomrule
    \end{tabular}
\end{table}



\textbf{W2: Sensitivity to Hyperparameters.} Besides, the paper doesn't thoroughly discuss the sensitivity of Ross to various hyperparameters, such as the denoising schedule or architecture choices. It would be beneficial to add this part analysis and show Ross's denoising part is robust and easy to train.


\textbf{A2:}
We appreciate the reviewer's suggestion to thoroughly discuss the sensitivity of Ross.
%
We study the effectiveness of different schedules of $\beta$ in the following table, where all methods are equipped with CLIP-VIT-L/14@336 and Qwen2-7B-Instruct.
%
The pre-training data is LLaVA-558K and the instruction tuning data is Cambrian-737K.
%
From the table, we can tell that even with different schedules of $\beta$, Ross \textit{consistently} improves the baseline, demonstrating its robustness to the denoising schedule.


\begin{table}[H]
    \centering\small
    % \caption{
    % Schedule. 558K+737K. CLIP-Qwen2-7B-Instruct.
    % %
    % \textbf{Convert to Figure when adding to the main paper!}
    % }
    % \label{tab:schedule}
    % \vspace{-5pt}
    \begin{tabular}{l llllll}
    \toprule
    Schedule of $\beta$ & POPE & Hallu. & MMVP & ChartQA & MMB$^{\text{EN}}$ \\
    \midrule
    -- & 87.9 & 55.0 & 29.6 & 34.0 & 73.8 \\
    
    Linear~\citep{ho2020denoising} & 88.1 \up{0.2} & 57.3 \up{2.3} & 42.0 \up{12.4} & 39.2 \up{5.2} & 75.1 \up{1.3} \\
    
    Scaled Linear~\citep{rombach2022high} & \textbf{88.4 \up{0.5}} & 58.3 \up{3.3} & 40.0 \up{10.4} & \textbf{40.7 \up{6.7}} & 75.3 \up{1.5} \\
    
    GLIDE Softmax~\citep{nichol2022glide} & \textbf{88.4 \up{0.5}} & \textbf{59.1 \up{4.1}} & \textbf{42.2 \up{12.6}} & 40.4 \up{6.4} & 75.2 \up{1.4} \\
    
    GeoDiff Sigmoid~\citep{xu2022geodiff} & 88.2 \up{0.3} & 57.7 \up{2.7} & 41.3 \up{11.7} & 38.9 \up{4.9} & \textbf{75.5 \up{1.7}} \\
    \bottomrule
    \end{tabular}
\end{table}


As for the architecture choices, we have analyzed the impact of different visual tokenizers.
%
The results, presented in Figure 10, show that the KL-16 tokenizer outperforms the VQ-16 tokenizer. 
%
One intuitive explanation is that KL-16 preserves more low-level details compared to VQ-16, as quantization can lead to information loss.
%
Additionally, Figure 10 highlights the importance of the self-attention module. 
%
Since the original visual outputs are causal, modeling inter-token dependencies via self-attention is crucial. 
%
The number of trainable parameters for the denoiser is not the primary factor affecting performance.


\textbf{Q1: Comparison with VQ-based LMMs.} This not be a major issue, but it's not very natural to see that using vision encoder to encode image pixels into LLM's embeddings and use another denosing module to reconstruct it back to image pixels. This may introduce improvements since the model better maintains the information of original images, but it may be more natural to see it‘s used in a quantized tokenizer based LMM like EMU-3 and Chamelon. I was wondering how the authors feel about this and have insights on this question?



\textbf{A3:}
The main reasons for not following VQ-based methods such as Emu-3 and Chameleon are the training efficiency and data requirements.
%
They often require extensive training with large amounts of caption data to achieve robust image-text alignment. 
%
Despite this, their comprehension capabilities can still lag behind (Chameleon) or just be comparable (Emu-3) to the LLaVA baseline. 
%
In contrast, LLaVA’s plug-in architecture is much more data-efficient.
%
This efficiency is crucial for practical applications with reasonable GPU requirements.
%
Therefore, we mostly follow LLaVA's settings and leverage a denoiser to recover the high-level LMM's features back to the pixel space, which may be a little bit unconventional.

The underlying insight driving our design is that \textit{high-level features from LMMs can be mapped into the pixel space}.
%
To support this claim, we fine-tune the denoiser to recover latent tokens from a frozen KL-16 conditioned on Ross-7B features on ImageNet-1K for only five epochs, where the denoiser manages to produce reasonable reconstruction results (please refer to Figure 9 in the revised manuscript).
%
This interesting finding demonstrates that Ross-7B features actually contain image details.
%
However, the two-layer MLP adopted by LLaVA may be insufficient to fully extract this inherent information, hence the need for an extra denoising module.



\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/recon.pdf}
    \vspace{-15pt}
    \caption{
    \textbf{Reconstruction results} on ImageNet-1K~\citep{deng2009imagenet} validation set.
    %
    For each tuple, we show the input image (left) and the reconstructed image (right).
    %
    We train a denoiser to recover latent tokens of KL-16 conditioned on Ross-7B features with only five epochs on ImageNet-1K~\citep{deng2009imagenet} training set.
    %
    Reasonable reconstruction results demonstrate that \textit{high-level features of Ross-7B can be projected into the pixel space.}
    }
    \label{fig:recon}
\end{figure}








\section{{To Reviewer tGMa (4)}}


We thank reviewer tGMa for the valuable time and constructive feedback. 
%
We are particularly grateful for your kind words about the paper being ``well-organized and easy to follow'' with a ``clear presentation of the key ideas.''
%
Your observation that ``a simple auxiliary loss can improve the performance of LMMs'' is very inspiring and aligns with our goals.
%
We have done our best to address your suggestions point-by-point in our response below.


\textbf{W1: About Novelty and Insight.} The proposed method lacks novelty and insight. As noted in Section 2, previous work (Emu-2), has explored using images as additional supervision in the form of generative objectives. Consequently, the contribution of this paper is limited, focusing mainly on a variation of established methods.

\textbf{A1:}
We would like to clarify that ``generation'' and ``reconstruction'' are fundamentally different approaches.
%
Previous works (Emu-2) explore ``generative objectives'', while our Ross is a kind of ``reconstructive objective''.
%
The detailed pipeline comparison can be found in Figure 11 in the Appendix.
%
Specifically, Emu-2 takes outputs corresponding to \textit{learnable queries} as conditions, while our Ross takes outputs corresponding to \textit{visual inputs}. 

Empirically, our Ross significantly outperforms Emu-2 in comprehension tasks, demonstrating the effectiveness of ``reconstruction'' over ``generation''.
%
Moreover, we have compared reconstruction and generation in Table 2, where using generative objectives actually fails to bring improvements over the baseline.
%
This empirical evidence highlights the effectiveness of the reconstructive approach over the generative one.

Both the distinct pipeline and the superior performance of Ross underscore our contributions and insights.




\textbf{W2: Risking the Langauge Capabilities.} The proposed method lack interpretability. While using pixel-level reconstruction as an auxiliary task may enhance fine-grained image recognition, this approach risks impairing the language capabilities of the multimodal model, as the final task output is high-level semantic language. The authors provide insufficient experiments and explanations regarding this trade-off, leaving questions about potential impacts on language performance.


\textbf{A2:}
Following suggestions, we evaluate multi-modal benchmarks that mainly require general knowledge following Cambrian-1, including ScienceQA, MMMU, and AI2D.
%
Furthermore, we incorporate representative language benchmarks, including general understanding on MMLU and HellaSwag, and instruction-following on IFEval.
%
Empirical results demonstrate that Ross does \textit{not} harm language capabilities as it brings improvements in most cases.



\begin{table}[H]
    \centering\small
    % \caption{
    % \textbf{Evaluations on language performance.}
    % %
    % We evaluate multi-modal benchmarks that mainly require general knowledge following~\cite{tong2024cambrian}.
    % %
    % Furthermore, we incorporate representative \textit{zero-shot} language benchmarks, including general understanding on MMLU~\citep{hendrycks2020measuring} and HellaSwag~\citep{zellers2019hellaswag}, and instruction-following on IFEval~\citep{zhou2023instruction}.
    % }
    % \label{tab:language}
    % \vspace{-5pt}
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{l rr rr rr rr}
    \toprule
    & \multicolumn{4}{c}{CLIP-ViT-L/14@336} & \multicolumn{4}{c}{SigLIP-ViT-SO400M/14@384} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    
    & \multicolumn{2}{c}{Vicuna-7B-v1.5} & \multicolumn{2}{c}{Qwen2-7B-Instruct} & \multicolumn{2}{c}{Vicuna-7B-v1.5} & \multicolumn{2}{c}{Qwen2-7B-Instruct} \\
    
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    Benchmark & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} \\
    
    \hline
    \rowcolor{lightgray}
    \multicolumn{9}{l}{\textit{Vision-Language Benchmarks on Knowledge}} \\
    
    
    ScienceQA$_{\text{test}}$ & 68.5 & \textbf{69.0 \up{0.5}} & 76.5 & \textbf{77.4 \up{0.9}} & 69.6 & \textbf{71.3 \up{1.7}} & 78.3 & \textbf{78.5 \up{0.2}} \\
    
    MMMU$_{\text{dev}}$ & 30.0 & \textbf{34.0 \up{4.0}} & 44.0 & \textbf{45.3 \up{1.3}} & 33.3 & \textbf{38.0 \up{4.7}} & 38.7 & \textbf{41.3 \up{2.6}} \\
    
    MMMU$_{\text{val}}$ & 35.3 & \textbf{36.0 \up{0.7}} & 41.9 & \textbf{42.6 \up{0.7}} & 34.2 & \textbf{35.4 \up{1.2}} & 41.8 & \textbf{43.8 \up{2.0}} \\
    
    AI2D$_{\text{test}}$ & 61.2 & \textbf{61.4 \up{0.2}} & 71.9 & \textbf{73.3 \up{1.4}} & \textbf{62.6} & 62.4 \down{0.2} & 74.0 & \textbf{74.5 \up{0.5}} \\
    
    \hline
    \rowcolor{lightgray}
    \multicolumn{9}{l}{\textit{Language Benchmarks}} \\
    
    MMLU & 26.5 & \textbf{27.4 \up{0.9}} & 57.1 & \textbf{60.7 \up{3.6}} & \textbf{26.0} & 25.9 \down{0.1} & 60.9 & \textbf{61.0 \up{0.1}} \\
    
    HellaSwag$_{\text{acc-norm}}$ & \textbf{27.0} & 26.9 \down{0.1} & \textbf{46.4} & 46.2 \down{0.2} & \textbf{27.1} & 27.0 \down{0.1} & 45.5 & \textbf{46.6 \up{1.1}} \\
    
    IFEval$_{\text{strict-inst}}$ & 41.2 & \textbf{44.6 \up{3.4}} & 47.1 & \textbf{49.2 \up{2.1}} & 43.6 & \textbf{43.8 \up{0.2}} & 47.8 & \textbf{48.1 \up{0.3}} \\
    
    IFEval$_{\text{strict-prompt}}$ & 28.7 & \textbf{35.3 \up{6.7}} & 35.1 & \textbf{37.0 \up{1.9}}  & 32.5 & \textbf{33.1 \up{0.6}} & 35.3 & \textbf{36.2 \up{0.9}} \\

    \cmidrule{1-9}
    Average & 39.8 & \textbf{41.8 \up{2.0}} & 52.5 & \textbf{54.0 \up{1.5}} & 41.1 & \textbf{42.1 \up{1.0}} & 52.8 & \textbf{53.8 \up{1.0}} \\
    
    \bottomrule
    \end{tabular}
\end{table}


\textbf{W3: Scalability.} The scalability of the empirical findings is uncertain. It remains unclear whether the optimal settings identified would hold in different scenarios or with variations in model scale, training data, and other factors. Although the authors attempt to address this concern with results in Table 3, these efforts are insufficient, as many relevant variables remain unexplored.

\textbf{A3:}
We appreciate the reviewer's insightful feedback regarding the scalability of our empirical findings.
%
To address these concerns, we have conducted additional experiments to study (1) the model scaling behavior and (2) the data scaling behavior of Ross.

(1) To study the stability and scalability of Ross across different model sizes, we use the Qwen2.5 series with varying sizes as the base language model while keeping the CLIP-ViT-L/14@336 as the visual encoder.
%
The pre-training data is LLaVA-558K, and the instruction tuning data is LLaVA-665K.
%
The results, shown in the following table, demonstrate that \textit{Ross consistently brings improvements over the baseline (LLaVA) across different model sizes}.

\begin{table}[H]
    \centering\footnotesize
    % \caption{
    % \textbf{Model scaling of \method.}
    % %
    % We take Qwen2.5 series~\citep{qwen2.5} as the base language model and CLIP-ViT-L/14@336~\citep{radford2021learning} as the visual encoder.
    % %
    % Pre-training data is LLaVA-558K~\citep{liu2023visual} and the instruction tuning data is LLaVA-665K~\citep{liu2024improved}.
    % }
    % \label{tab:model_scale}
    % \vspace{-5pt}
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{l rr rr rr rr}
    \toprule
    \multirow{2}{*}{Benchmark} & \multicolumn{2}{c}{0.5B} & \multicolumn{2}{c}{1.5B} & \multicolumn{2}{c}{3B} & \multicolumn{2}{c}{7B} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} \\
    \midrule
    
    POPE$_{\text{acc}}$ & 50.0 & \textbf{60.4 \up{10.4}} & 85.3 & \textbf{87.9 \up{2.4}} & 87.3 & \textbf{88.1 \up{0.8}} & 87.9 & \textbf{88.4 \up{0.5}} \\
    
    HallusionBench$_{\text{aAcc}}$ & 45.8 & \textbf{48.0 \up{2.2}} & 48.7 & \textbf{49.6 \up{0.9}} & 52.2 & 52.2 \textcolor{mygray}{-- 0.0} & 48.7 & \textbf{53.7 \up{5.0}} \\
    
    MMBench-EN$_{\text{dev}}$ & 55.2 & \textbf{60.4 \up{5.2}} & 67.5 & \textbf{68.2 \up{1.7}} & 70.6 & \textbf{71.4 \up{0.8}} & 75.0 & \textbf{75.7 \up{0.7}} \\
    
    MMBench-CN$_{\text{dev}}$ & 45.6 & \textbf{48.9 \up{3.3}} & 62.4 & \textbf{63.9 \up{1.5}} & 68.0 & \textbf{69.1 \up{1.1}} & \textbf{73.6} & 73.5 \down{0.1} \\
    
    SEED$_{\text{img}}$ & \textbf{55.8} & 55.6 \down{0.2} & 66.3 & \textbf{66.8 \up{0.5}} & 68.2 & \textbf{68.4 \up{0.2}} & 70.6 & \textbf{71.0 \up{0.4}} \\
    
    OCRBench & 229 & \textbf{248 \up{19}} & 291 & \textbf{298 \up{7}} & \textbf{313} & 308 \down{5} & 334 & \textbf{358 \up{24}} \\
    
    MMMU$_{\text{dev}}$ & 35.2 & \textbf{36.0 \up{0.8}} & 44.7 & \textbf{45.0 \up{0.3}} & 48.7 & \textbf{49.0 \up{0.3}} & 48.0 & 48.0 \textcolor{mygray}{-- 0.0} \\
    
    MMMU$_{\text{val}}$ & 38.0 & \textbf{40.3 \up{1.7}} & 41.8 & \textbf{43.6 \up{1.8}} & 41.6 & \textbf{42.7 \up{1.1}} & 47.3 & \textbf{48.0 \up{0.7}} \\
    
    AI2D$_{\text{test}}$ & 45.3 & \textbf{46.0 \up{0.7}} & 59.0 & \textbf{59.5 \up{0.5}} & 62.9 & \textbf{63.2 \up{0.3}} & 68.3 & \textbf{68.5 \up{0.2}} \\
    
    RealWorldQA & 45.1 & \textbf{46.4 \up{1.3}} & 50.5 & \textbf{53.5 \up{3.0}} & 55.7 & \textbf{57.9 \up{2.2}} & 59.5 & \textbf{59.9 \up{0.4}} \\

    \cmidrule{1-9}
    Average & 43.9 & \textbf{46.7 \up{2.8}} & 55.3 & \textbf{56.8 \up{1.5}} & 58.9 & \textbf{59.3 \up{0.4}} & 61.2 & \textbf{62.3 \up{1.1}} \\
    
    \bottomrule
    \end{tabular}
\end{table}


(2) Next, to study the impact of the training data scale, we used Qwen2-7B-Instruct as the base language model and CLIP-ViT-L/14@336 as the visual encoder.
%
We compared the performance of Ross and the baseline under different scales of training data.
%
The following table demonstrates that \textit{Ross consistently brings significant improvements as the training data scale increases.}


\begin{table}[H]
    \centering\small
    % \caption{
    % \textbf{Data scaling of \method.}
    % %
    % We take Qwen2-7B-Instruct~\citep{yang2024qwen2} as the base language model and CLIP-ViT-L/14@336~\citep{radford2021learning} as the visual encoder.
    % }
    % \label{tab:data_scale}
    \vspace{-5pt}
    \begin{tabular}{llc llllll}
    \toprule
    PT & SFT & $\mathcal{L}_{\mathrm{LMM}}^{\mathrm{visual}}$ & POPE & Hallu. & ChartQA & OCRBench & MMB$^{\text{EN}}$ & AI2D \\
    
    \midrule
    \multirow{2}{*}{558K} & \multirow{2}{*}{737K} & -- & 87.9 & 55.0 & 34.0 & 363 & 73.8 & 72.4 \\
    & & \checkmark & \textbf{88.4 \up{0.5}} & \textbf{59.1 \up{4.1}} & \textbf{40.4 \up{6.4}} & \textbf{380 \up{17}} & \textbf{75.2 \up{1.4}} & \textbf{73.3 \up{0.9}} \\

    \midrule
    \multirow{2}{*}{558K} & \multirow{2}{*}{1.2M} & -- & 88.5 & 57.3 & 37.0 & 389 & 75.7 & 74.5 \\
    & & \checkmark & \textbf{88.8 \up{0.3}} & \textbf{57.8 \up{0.5}} & \textbf{42.0 \up{5.0}} & \textbf{392 \up{3}} & \textbf{76.8 \up{1.1}} & \textbf{74.7 \up{0.2}} \\

    \midrule
    \multirow{2}{*}{2M} & \multirow{2}{*}{737K} & -- & 88.1 & 55.6 & 37.3 & 384 & 76.2 & 72.3 \\
    & & \checkmark & \textbf{88.3 \up{0.2}} & \textbf{56.2 \up{0.6}} & \textbf{41.9 \up{4.5}} & \textbf{398 \up{14}} & \textbf{77.0 \up{0.8}} & \textbf{73.4 \up{1.1}} \\

    \midrule
    \multirow{2}{*}{2M} & \multirow{2}{*}{1.2M} & -- & 88.5 & 53.8 & 41.2 & 388 & 76.5 & 73.9 \\
    & & \checkmark & \textbf{88.9 \up{0.4}} & \textbf{57.3 \up{2.5}} & \textbf{43.2 \up{2.0}} & \textbf{405 \up{17}} & \textbf{78.0 \up{1.5}} & \textbf{74.1 \up{0.2}} \\
    
    \bottomrule
    \end{tabular}
\end{table}

These additional experiments provide a more comprehensive understanding of the scalability of Ross. 
%
They show that the model's performance improvements are not limited to specific configurations but hold across different model sizes and training data scales.
%
The robustness and consistency of these results suggest that Ross is a reliable and scalable solution for multimodal tasks.


\textbf{Q1: Ross-13B performs consistently worse than Ross-7B.} The results in Table 4 appear counter-intuitive, as Ross-13B performs consistently worse than Ross-7B. This raises concerns about whether the proposed method is well-suited to larger-scale models. Clarification on this disparity and potential scalability issues would strengthen the paper.


\textbf{A4:}
We would like to clarify that the performance of LMMs largely depends on the base LLM. 
%
In our experiments, Ross-13B is based on Vicuna-13B-v1.5, while Ross-7B is based on Qwen2-7B-Instruct, which is a much stronger LLM backbone.
%
This difference in base models can explain why Ross-13B performs worse than Ross-7B.
%
Similar issues have been observed in other methods. 
%
For example, Cambrian-1-13B performs worse than Cambrian-1-8B in most cases because the former uses Vicuna-13B-v1.5, while the latter uses Llama3-8B-Instruct.

To further investigate this issue, we conducted additional experiments using Vicuna-v1.5 series as the language model while keeping the training data the same, resulting in Ross-7B$_{\text{vicuna}}$ and Ross-13B$_{\text{vicuna}}$, respectively.
%
Empirical results demonstrate that Ross-13B$_{\text{vicuna}}$ significantly outperforms Ross-7B$_{\text{vicuna}}$.
%
This indicates that Ross is indeed well-suited to larger-scale models when the base language models are comparable.


\begin{table}[H]
    \centering\small
    % \caption{
    % \textbf{Comparison under the same base language model.}
    % %
    % $^\ddag$We evaluate the official checkpoint using VLMEvalKit~\citep{duan2024vlmevalkit}.
    % }
    % \vspace{-5pt}
    \setlength{\tabcolsep}{2.5pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{r lllllllll}
        \toprule
        Model & POPE & Hallu. & MMB$^\text{EN}$ & MMB$^\text{CN}$ & SEED$^\text{I}$ & MMMU & MMVP & GQA & AI2D \\
        
        \hline
        \rowcolor{lightgray}
        \multicolumn{10}{l}{\textit{Base LLM: Vicuna-7B-v1.5}} \\
        
        LLaVA-v1.5-7B$^\ddag$ \citep{liu2024improved} & 86.2 & 47.5 & 65.5 & 58.5 & 66.0 & 34.4 & 20.0 & 62.0 & 55.4 \\
        LLaVA-v1.6-7B$^\ddag$ \citep{liu2024llavanext} & 86.5 & 35.8 & 67.4 & 60.1 & \textbf{70.2} & 35.8 & 37.3 & \textbf{64.2} & 67.1 \\

        \textbf{\method-7B}$_{\text{vicuna}}$ & \textbf{88.2} & \textbf{55.2} & \textbf{67.7} & \textbf{61.3} & 67.6 & \textbf{36.9} & \textbf{39.3} & 63.7 & \textbf{69.3} \\
        
        \hline
        \rowcolor{lightgray}
        \multicolumn{10}{l}{\textit{Base LLM: Vicuna-13B-v1.5}} \\
        LLaVA-v1.5-13B$^\ddag$ \citep{liu2024improved} & 82.5 & 44.9 & 68.8 & 63.6 & 68.2 & 36.6 & 31.9 & 63.3 & 60.8 \\
        LLaVA-v1.6-13B$^\ddag$ \citep{liu2024llavanext} & 86.2 & 36.7 & 70.0 & 64.1 & 71.9 & 36.2 & 35.6 & \textbf{65.4} & 72.4 \\
        % InternVL-13B \citep{chen2024internvl} & 87.1 & ? & ? & ? & ? & ? & ? & 63.9 & ? & ? \\
        Mini-Gemini-13B \citep{li2024mini} & -- & -- & 68.6 & -- & 73.2 & 37.3 & 19.3 & 63.7 & 70.1 \\
        Cambrian-1-13B \citep{tong2024cambrian} & 85.7$^\ddag$ & 54.0$^\ddag$ & \textbf{75.7} & 65.9$^\ddag$ & \textbf{74.4} & 40.0 & 41.3 & 64.3 & 73.6 \\
        
        \textbf{\method-13B}$_{\text{vicuna}}$ & \textbf{88.7} & \textbf{56.4} & 73.6 & \textbf{67.4} & 71.1 & \textbf{41.3} & \textbf{44.7} & 65.2 & \textbf{73.8} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:13b}
    \vspace{-10pt}
\end{table}


\textbf{Q2: Further Elaborations.} The analysis in Section 5.2 is unclear. My understanding is that the authors aim to demonstrate that additional visual supervision enables the model to better focus on relevant areas of the image during VQA tasks. However, the reasoning behind this effect is not well-explained. Further elaboration on the mechanisms or evidence supporting this claim would enhance interpretability.


\textbf{A5:}
To better explain the reasoning behind how the vison-centric supervision enables the model to focus on relevant areas of the image during VQA tasks, we provide qualitative comparison using GradCAM~\citep{selvaraju2020grad} on MMVP~\citep{tong2024eyes}, since GradCAM helps in understanding which parts of the image the model is focusing on, making the model's decision-making process more transparent.
%
Please refer to Figure 12 in Appendix C.2.
%
Specifically, it works by computing the gradients of the target class with respect to the feature maps in a specific layer of the network, typically the last convolutional layer for CNNs. 
%
These gradients are then weighted and summed to produce a heat map that highlights the regions of the input image that are most important for the prediction.


In our analysis, we visualize the gradient of the second-to-last block of the LMM, regarding the option of the ground-truth answer as the target class.
%
Specifically in this case, where the providing question is about the spider web, our proposed vision-centric supervision signals provide more reasonable gradients and urge LMMs to focus on relevant regions, \textit{i.e.}, the spider web, as the training evolves.


\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{images/gradcam_steps.pdf}
    \vspace{-5pt}
    \caption{
    \textbf{Qualitative results using GradCAM~\citep{selvaraju2020grad}} on MMVP~\citep{tong2024eyes}.
    %
    We visualize the gradient of the second-to-last block of the LMM using the option of the ground-truth answer as the target class.
    %
    Equipped with our proposed vision-centric supervision signals, \method provides more reasonable gradients and urges LMMs to focus on relevant regions (the spider web) as the training evolves.
    }
    \label{fig:gradcam}
\end{figure}



















\section{{To Reviewer rXNr (5)}}

We thank reviewer rXNr for the valuable time and constructive feedback. 
%
We appreciate your comments on the paper being ``well-organized and easy to read'' and the ``straightforward'' motivation.
%
In the following, we have done our best to address your suggestions point-by-point.


\textbf{W1: About the Novelty.} The novelty is somewhat incremental. Utilizing image supervision is a very straightforward idea, and can be implemented by various ways. Denoising-based reconstruction is a very well-developed strategy in the field of image diffusion/generation. There is no specific in-depth design in the proposed architecture.

\textbf{A1:}
We would like to emphasize that our main contribution is proposing a novel vision-centric supervision for enhanced comprehension capabilities for LMMs, instead of any specific technical modules.
%
The underlying motivation is input images themselves inherently provide rich and detailed information, which is quite important for fine-grained comprehension tasks.
%
As a result, we regard LMMs reconstructing input images as the supervision of those visual outputs.


Actually, Reviewer kvNb uses ``novel image-based supervision'' to describe our work.
%
Reviewer MCFE regards our work as a ``step forward''.
%
Reviewer SsLG says this paper is ``very novel'', and Reviewer tGMa thinks our work is ``inspiring''.



(1) The idea is not trivial. 
%
While utilizing image supervision may \textit{seem} straightforward, effectively using images to produce meaningful feedback through reconstruction for LMMs remains largely unexplored. 
%
\textit{The key challenge lies in handling the heavy spatial redundancy of natural visual signals.}
%
To address this, we systematically explore various reconstruction targets and objectives, which are definitely specific in-depth designs aimed at enhancing the comprehension capabilities of LMMs. 
%
Moreover, the self-attention module of the denoiser is specifically designed to manage the causal dependencies in the original visual outputs, ensuring that the model can effectively process and understand the whole visual content.

(2) Our contribution is not a newly introduced denoising strategy.
%
While denoising is a well-developed strategy in the field of image \textit{generation}, we are the first to leverage the denoising objective as a \textit{reconstruction} method to \textit{boost fine-grained comprehension for LMMs}. 
%
Furthermore, denoising is just one type of objective under our framework.
%
We adopt denoising simply because it alleviates the redundancy of natural visual signals. 
%
In fact, as demonstrated in Figure 7, vanilla regression still brings significant improvements, highlighting the flexibility and effectiveness of our approach.




\textbf{W2: When Does the Inherent Details Become Important?} The authors claim that the proposed method capitalizes on the inherent richness and detail present within input images themselves, which are often lost in pure text supervision. In which cases, the information within the image is important? The authors should provide a more detailed analysis of this aspect. Is this information crucial for all common cases?



\textbf{A2:}
We extend ablations to more representative benchmarks, where Ross manages to bring improvements in most cases.
%
By systematically analyzing the results, we find the improvements are more significant on fine-grained comprehension benchmarks such as HallusionBench, MMVP, ChartQA, and OCRBench, as visual contents for these benchmarks are more crucial. 
%
In contrast, observed by~\cite{tong2024cambrian}, LMMs can sometimes correctly answer the question without providing the image on knowledge benchmarks such as MMMU and AI2D, where the improvements seem to be less significant.


\begin{table}[H]
    \centering\footnotesize
    % \caption{
    % \textbf{Extended ablations.}
    % }
    % \label{tab:complete_abl}
    \vspace{-5pt}
    \setlength{\tabcolsep}{3pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l rr rr rr rr}
    \toprule
    & \multicolumn{4}{c}{CLIP-ViT-L/14@336} & \multicolumn{4}{c}{SigLIP-ViT-SO400M/14@384} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    & \multicolumn{2}{c}{Vicuna-7B-v1.5} & \multicolumn{2}{c}{Qwen2-7B-Instruct} & \multicolumn{2}{c}{Vicuna-7B-v1.5} & \multicolumn{2}{c}{Qwen2-7B-Instruct} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    Benchmark & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} & LLaVA & \multicolumn{1}{c}{Ross} \\
    \midrule
    
    POPE$_{\text{acc}}$ & 86.3 & \textbf{87.2 \up{0.9}} & 87.9 & \textbf{88.4 \up{0.5}} & 86.0 & \textbf{87.7 \up{1.7}} & 88.5 & \textbf{88.7 \up{0.2}} \\
    
    HallusionBench$_{\text{aAcc}}$ & 52.5 & \textbf{55.8 \up{3.3}} & 55.0 & \textbf{59.1 \up{4.1}} & 50.4 & \textbf{53.8 \up{3.4}} & 57.3 & \textbf{58.2 \up{0.9}} \\
    
    MMBench-EN$_{\text{dev}}$ & 67.0 & \textbf{67.6 \up{0.6}} & 73.8 & \textbf{75.2 \up{1.4}} & 64.5 & \textbf{69.2 \up{4.7}} & 76.3 & \textbf{76.9 \up{0.6}} \\
    
    MMBench-CN$_{\text{dev}}$ & \textbf{60.0} & 59.5 \down{0.5} & 72.9 & \textbf{73.7 \up{0.8}} & 63.1 & \textbf{63.4 \up{0.3}} & 75.7 & \textbf{76.3 \up{0.7}} \\
    
    SEED$_{\text{img}}$ & \textbf{66.7} & 66.4 \down{0.3} & 70.3 & \textbf{70.7 \up{0.4}} & 68.2 & \textbf{69.0 \up{0.8}} & \textbf{72.3} & 72.1 \down{0.2} \\
    
    MMMU$_{\text{dev}}$ & 30.0 & \textbf{34.0 \up{4.0}} & 44.0 & \textbf{45.3 \up{1.3}} & 33.3 & \textbf{38.0 \up{4.7}} & 38.7 & \textbf{41.3 \up{2.6}} \\
    
    MMMU$_{\text{val}}$ & 35.3 & \textbf{36.0 \up{0.7}} & 41.9 & \textbf{42.6 \up{0.7}} & 34.2 & \textbf{35.4 \up{1.2}} & 41.8 & \textbf{43.8 \up{2.0}} \\
    
    MMVP & 28.0 & \textbf{36.3 \up{8.3}} & 29.6 & \textbf{42.2 \up{12.6}} & 27.3 & \textbf{38.0 \up{10.7}} & 40.7 & \textbf{49.3 \up{8.6}} \\
    
    AI2D$_{\text{test}}$ & 61.2 & \textbf{61.4 \up{0.2}} & 71.9 & \textbf{73.3 \up{1.4}} & \textbf{62.6} & 62.4 \down{0.2} & 74.0 & \textbf{74.5 \up{0.5}} \\
    
    ChartQA$_{\text{test}}$ & 32.9 & \textbf{39.8 \up{6.9}} & 36.2 & \textbf{41.6 \up{5.4}} & 34.0 & \textbf{48.2 \up{14.2}} & 44.4 & \textbf{46.9 \up{2.5}} \\
    
    DocVQA$_{\text{val}}$ & 33.4 & \textbf{41.6 \up{8.2}} & 31.1 & \textbf{44.7 \up{13.6}} & 40.4 & \textbf{40.7 \up{0.3}} & 39.2 & \textbf{39.3 \up{0.1}} \\
    
    InfoVQA$_{\text{val}}$ & 21.2 & \textbf{26.4 \up{5.2}} & 22.1 & \textbf{39.3 \up{16.2}} & 22.8 & \textbf{23.3 \up{0.5}} & 24.0 & \textbf{25.1 \up{1.1}} \\
    
    TextVQA$_{\text{val}}$ & 55.7 & \textbf{58.7 \up{3.0}} & 52.0 & \textbf{54.1 \up{2.1}} & 60.5 & \textbf{62.6 \up{2.1}} & 56.3 & \textbf{57.5 \up{1.2}} \\
    
    OCRBench & 339 & \textbf{350 \up{11}} & 363 & \textbf{381 \up{18}} & 354 & \textbf{365 \up{11}} & 432 & \textbf{448 \up{16}} \\
    
    RealWorldQA & 52.7 & \textbf{53.2 \up{0.5}} & 56.7 & \textbf{57.4 \up{0.7}} & 55.0 & \textbf{57.1 \up{2.1}} & 57.9 & \textbf{59.1 \up{1.2}} \\

    \cmidrule{1-9}

    Average & 47.8 & \textbf{50.6 \up{2.8}} & 52.1 & \textbf{56.4 \up{4.3}} & 49.2 & \textbf{52.4 \up{3.2}} & 55.4 & \textbf{56.9 \up{1.5}} \\
    
    \bottomrule
    \end{tabular}}
\end{table}


Examples in Figure 15 are vivid illustrations. 
%
Taking a close look at the given image becomes important to answer the question.
%
Under such cases, vision-centric supervision enables LMMs to pay more attention to visual content, thereby enhancing overall performance.



\textbf{W3: About Complexity and Efficiency.} No experiments on complexity and efficiency. Of course, utilizing more self-supervision loss can definitely improve the model's performance. However, this image-aware training may cost more time and GPU memories compared to previous text-only supervision. The authors should provide an in-depth analysis of complexity and efficiency for fair comparison.

\textbf{A3:}
We apologize for the oversight in quantifying and discussing the computational overhead.
%
To address this concern, we have conducted additional experiments to measure the computational costs and provide a clearer understanding of the practical trade-offs.
%
Evaluations are conducted using 8 A100 GPUs with a global batch size of 128.
%
Due to the limited GPU memory, we accumulate 4 gradient steps and the batch size per GPU is 4.
%
The whole stage requires 5757 training steps.
%
GPU memories are averaged over 8 GPUs with DeepSpeed Zero 3.
%
As demonstrated in the following table, Ross introduces a negligible increase in training time and GPU memory.



\begin{table}[H]
    \centering\small
    \vspace{-5pt}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{ll c lllll}
    \toprule
    Vision & Base LLM & $\mathcal{L}_{\mathrm{LMM}}^{\mathrm{visual}}$ & \begin{tabular}[c]{@{}l@{}}Trainable\\ Parameters\end{tabular} & Speed (s/iter) & Time & \begin{tabular}[c]{@{}l@{}}GPU\\ Memory\end{tabular} \\
    \midrule
    CLIP-L/336 & Qwen2-7B-Instruct & -- & 7.63 B & 8.31 & 13h 17min & 45.34 G \\
    CLIP-L/336 & Qwen2-7B-Instruct & \checkmark & 7.68 B & 9.02 (1.09$\times$) & 14h 25min & 46.62 G (1.03$\times$) \\

    CLIP-L/336 & Vicuna-13B-v1.5 & -- & 13.05 B & 13.33 & 21h 19min & 48.62 G \\
    CLIP-L/336 & Vicuna-13B-v1.5 & \checkmark & 13.11 B & 14.69 (1.10$\times$) & 23h 30min & 49.07 G (1.01$\times$) \\

    \midrule

    SigLIP-L/384 & Qwen2-7B-Instruct & -- & 7.63 B & 8.77 & 14h 1min & 47.08 G \\
    SigLIP-L/384 & Qwen2-7B-Instruct & \checkmark & 7.68 B & 9.48 (1.08$\times$) & 15h 9min & 52.07 G (1.11$\times$) \\

    SigLIP-L/384 & Vicuna-13B-v1.5 & -- & 13.05 B & 14.22 & 22h 44min & 48.80 G \\
    SigLIP-L/384 & Vicuna-13B-v1.5 & \checkmark & 13.11 B & 15.32 (1.08$\times$) & 24h 30min & 52.68 G (1.08$\times$) \\
    \bottomrule
    \end{tabular}
\end{table}


\textbf{W4:} Given an image-text pair input, just some of the image-based contents are aligned with the text. I do not see any text-guided image reconstruction design in the architecture. This may help reduce the redundancy contexts.

\textbf{A4:}
We understand the reviewer's concern regarding the alignment of image-based content with the text.
%
In fact, our Ross performs \textit{vanilla} reconstruction instead of text-guided reconstruction.
%
This is because the visual tokens are always processed before the text instructions (as shown in Figure 2), and the causal nature of LLMs means visual tokens does \textit{not} interact with text inputs.


We would like to clarify that the reconstructive pretext task does not aim to an enhanced image-text alignment directly.
%
Instead, its primary goal is to mine the inherent information in the input images that might be overlooked by sparse text instructions.
%
By reconstructing the images, the model can extract more comprehensive visual features, providing a richer context that allows the LMMs to decide which aspects to focus on based on the subsequent text instructions.
%
As a result, this approach contributes to better fine-grained comprehension of the full contents of the input images.




{\small
\bibliographystyle{iclr2025_conference}
\bibliography{ref}
}
